GOSPAL: An Efficient Strategy-Proof mechanism for Constrained Resource Allocation

We consider allocation of a resource to multiple interested users with a constraint that if the resource is allocated to user $i$ then it can not be allocated simultaneously to a predefined set of users $\cS_i$ . This scenario arises in many practical systems that include wireless networks and constrained queuing systems. It is known that socially optimal strategy-proof mechanism is not only NP-hard, but it is also hard to approximate. This renders optimal policy hard to use in practice. Here, we propose a computationally efficient mechanism and prove it to be strategy proof. Using Monte Carlo simulations, we show that the social utility of the proposed scheme is close to that of the optimal. Further, we demonstrate how the proposed mechanism can be used for fair and efficient short-term spectrum allocation in resource constrained large wireless networks.

==> introduction.tex <==
\section{Introduction}
Optimal use of resources has always been a concern. In today\textquoteright s
world with increasing demand, efficient use of limited and scarce
resource has become a challenge. A resource allocation mechanism
must be designed to meet the strategic goals of the system. The
desired strategic goals may include maximization of social welfare,
efficient and fair utilization of limited resource and maximization of
revenue. Auction based mechanism is a popular way of distributing
the available resource among users \cite{krishna2009auction}.Here, it is assumed that each
user has some quantitative valuation of the usefulness of the resource
for them. Based on the valuation, users bid for the resource and the
auctioneer or centralized controller arbitrates resource distribution based
on the received bid values. Each user is assumed to be greedy
and rational. Hence, a key challenge in using auctions for resource
distribution is that the users may not bid their true valuation if that
benefits them. Hence, key challenge in this approach is to device a
strategy-proof/truthful auction in which users do not have any incen-
tive in not bidding their true valuation \cite{osborne1994course}.
Hence, being rational, their bids would equal their respective true valuations. A well known
Vickrey Clarke Grooves (VCG) auction provides a framework for
designing strategy proof mechanism that maximizes social utility
 \cite{vickrey1961counterspeculation,clarke1971multipart,groves1973incentives}. However, depending on scenario under consideration
VCG may not be computationally feasible. Thus, alternative ways
are required.

\par In this paper, we consider a constrained resource allocation prob-
lem in which a single resource can be allocated to multiple interested
users. Users are assumed to be selfish and rational. The allocation is
constrained in a sense that corresponding to each user $i$, there exists
a pre-specified set of users $\cS_i$ such that if the resource is given to
user $i$, then it can not be given to any user in $\cS_i$. This constrained
resource allocation is relevant in many applications including sched-
uling in ad-hoc networks, overlay device-to-device communication
and spectrum allocation in cellular networks. Moreover, in many of
these scenarios the resource in allocated for some time after which
the reallocation is done, e.g. a channel is allocated to non-interfering
links in wireless network for a predefined time slot and the allocation
may vary from slot to slot based on many factors including backlog,
delay, data priority and channel state. Thus, we assume that the
resource is auctioned periodically. It is known that VCG auction is
NP-hard for constrained resource allocation \cite{garey2002computers}. Thus, it can not be
used it this case as resource allocation needs to be computationally
fast for repeated execution.

\par In many applications for which the aforementioned constrained
auction mechanism is relevant, there are desirable features other than
maximization of social welfare for an allocation mechanism. For
example, if we consider each user $i$ to be a Base Station (BS) in a
cellular system and  $\cS_i$  to be the set BSs that interfere with $i$, then
for efficient utilization of the scarce and expensive spectrum must
be ensured. Thus, the number of BSs that get the spectrum may also
be important. Also, in the case where BSs may belong to different
operators, it is possible that \textquotedblleft small\textquotedblright operators may not be able to
bid comparatively with \textquotedblleft big\textquotedblright operators and hence may never get the
spectrum. It may be desirable to make the auction based allocation
fair in a sense that fraction of time slots in which the BSs get the
spectrum must be balanced across the BSs.{\it Our aim in this paper is
to propose a strategy-proof and computationally feasible auction for
resource allocation for constrained resource allocation problem. We
show that the proposed mechanism not only achieve near-optimal social utility
but also perform well in terms of resource utilization
and fairness parameters.}

Now, we state some most relevant previous work for the prob-
lem under consideration. A comprehensive overview of the game
theoretic approaches used for spectrum sharing in cognitive radio
networks is given in \cite{ji2007cognitive}.



%===============================================================================


In this paper, we consider a repeated constrained resource allocation problem in which a single resource can be
allocated to multiple interested users. Users are assumed to be selfish and rational. 
The allocation is constrained in a sense that corresponding to
each user $i$, there exists a pre-specified set of users $\cS_i$ such that if the resource is
given to user $i$, then it can not be given to any user in $\cS_i$. This constrained resource allocation 
is relevant in many applications including scheduling in ad-hoc networks, overlay device-to-device communication
and spectrum allocation in cellular networks. 
The allocation is for a limited time duration, referred to as {\it allocation frame} in sequel, and it is re-computed periodically.
In these settings, a well known strategy proof social utility optimal
auction  Vickrey Clarke Grooves (VCG) mechanism can be used for resource
allocation in each allocation frame \cite{vickrey1961counterspeculation,clarke1971multipart,groves1973incentives}.
However, we show that VCG mechanism in NP-hard and hence computationally
infeasible to implement. In \cite{myerson}, it is proved that if any resource allocation rule follows monotonicity behavior \cite{krishna2009auction}, then 
there exists a unique pricing scheme for which the resource allocation mechanism is strategy-proof. 
%
%
To address this, computationally efficient strategy-proof 
alternatives that include greedy \cite{zhou2008ebay} and SMALL \cite{wu2011small} are proposed. While SMALL has poor resource utilization, greedy suffers from
unfair allocation. In \cite{trust} authors propose a double auction based spectrum allocation  mechanism which holds strategy-proof property. Authors in \cite{gopinathan} propose spectrum allocation mechanism for repeated auctions for maximizing the social welfare. They also ensure fairness in spectrum allocation among the users.

To address these lacunae in the existing schemes, we propose an 
auction mechanism called Group Optimal Strategy-Proof Allocation (GOSPAL) and
show that it can be implemented in computationally efficient manner for
large number of users when when the maximum size of constrain sets $\cS_i$'s
is small. 

Some other relevant work includes the algorithms for real time dynamic spectrum allocation among the base station \cite{gandhi2008towards,subramanian2008near}. These algorithms are not strategy-proof \cite{osborne1994course}. Auction based general framework for spectrum allocation in cognitive network has been proposed by the authors in \cite{kasbekar}.
Authors in \cite{ji2007cognitive} propose auction based approach is efficient for spectrum allocation among the base stations in cognitive networks. Authors in \cite{matinmikko2014spectrum} present Licensed Shared Access framework for spectrum sharing between incumbent and secondary users. This framework requires efficient mechanism to address dynamic load variations of network.

{\bf Our main contributions are as follows:}
\begin{itemize}
	\item We study the problem of resource allocation among multiple users with limited constrained set, which is NP-Hard and becomes intractable for large set of users.
	\item We propose truthful mechanism Group Optimal Strategy-Proof Allocation (GOSPAL) for resource allocation in generic framework and also present its application in resource allocation among the base stations in wireless networks.
	\item With simulations we demonstrate that the proposed mechanism performs well in terms of achieving the social efficiency of resource allocation close to the optimal solution. The proposed mechanism is also computationally efficient, which makes it practical feasible for implementations in the large set of users.
\end{itemize}

The rest of the paper is organized as follows. Section \ref{sec:sys_model} describes the system model and problem formulation. In Section \ref{sec:algo}, proposed algorithm GOSPAL is presented in detail. We demonstrate the applicability of the proposed algorithm in spectrum allocation in wireless networks in Section \ref{sec:application}. Simulations results are presented in Section \ref{sec:Simulation}.In Section \ref{sec:conclusion} we conclude our work.






